Descriptor: Face Detection Dataset for Programmable Threshold-Based Sparse-Vision

Smart focal-plane and in-chip image processing has emerged as a crucial technology for vision-enabled embedded systems with energy efficiency and privacy. However, the lack of special datasets providing examples of the data that these neuromorphic sensors compute to convey visual information has hindered the adoption of these promising technologies. Neuromorphic imager variants, including event-based sensors, produce various representations such as streams of pixel addresses representing time and locations of intensity changes in the focal plane, temporal-difference data, data sifted/thresholded by temporal differences, image data after applying spatial transformations, optical flow data, and/or statistical representations. To address the critical barrier to entry, we provide an annotated, temporal-threshold-based vision dataset specifically designed for face detection tasks derived from the same videos used for Aff-Wild2. By offering multiple threshold levels (e.g., 4, 8, 12, and 16), this dataset allows for comprehensive evaluation and optimization of state-of-the-art neural architectures under varying conditions and settings compared to traditional methods. The accompanying tool flow for generating event data from raw videos further enhances accessibility and usability. We anticipate that this resource will significantly support the development of robust vision systems based on smart sensors that can process based on temporal-difference thresholds, enabling more accurate and efficient object detection and localization and ultimately promoting the broader adoption of low-power, neuromorphic imaging technologies. To support further research, we publicly released the dataset at \url{https://dx.doi.org/10.21227/bw2e-dj78}.

==> conclusion.tex <==
\section*{Conclusion}
\label{sec:conclusion}
Conventional high-resolution imaging suffers from energy and bandwidth issues due to the back-and-forth frame-by-frame data transfer of sensor and neural networks. Event sensors reduce these bottlenecks by introducing event-vision. However, the need for open-source event data, in particular, human face data with annotations, is one of the major bottlenecks in event-vision research. Besides, generating event data for faces is a challenging task. In this paper, we overcome this event data issue by proposing a programmable, digital threshold-based event dataset considering four thresholds (i.e., 4, 8, 12, and 16). 

In addition to the thresholded datasets, a threshold-based smart event generation algorithm was presented to generate desired
thresholded datasets. The tool flow will enable more research in event-vision. %In this paper, we also discussed the existing neural architectures for object detection and localization. 
We verified the effectiveness of our data using existing YOLO-v4, EfficientDet-b0, and MobileNets-v1 object detection and localization models. All three architectures achieve excellent AP50, 95.05\%, 98.08\%, and 96.69\% for YOLO-v4, EfficientDet-b0, and MobileNets-v1, respectively using the same threshold
= 8 valued dataset.
\vspace{-0.60cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Dummy%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



